Chance-Constrained Motion Planning with Event-Triggered Estimation

We consider the problem of autonomous navigation using limited information from a remote sensor network. Because the remote sensors are power and bandwidth limited, we use event-triggered (ET) estimation to manage communication costs. We introduce a fast and efficient sampling-based planner which computes motion plans coupled with ET communication strategies that minimize communication costs, while satisfying constraints on the probability of reaching the goal region and the point-wise probability of collision. We derive a novel method for offline propagation of the expected state distribution, and corresponding bounds on this distribution. These bounds are used to evaluate the chance constraints in the algorithm. Case studies establish the validity of our approach, demonstrating fast computation of optimal plans.

==> sections/Analysis.tex <==
\qh{Show probabilistic completeness, correctness, w.r.t. bounds}
\qh{hopefully optimality w.r.t. bounds}

% \subsection{Asymptotic Optimality}

In this section, we show that ET-GBT is sound and probabilistically complete with respect to the conservative upper bound, and satisfies the condition for asymptotic (near-)optimality of sampling-based tree search planners that sample the control space, such as SST or SST*.

\subsection{Probabilistic Completeness}

\begin{lemma}[Correctness]
    Upper bound...
\end{lemma}
\begin{proof}[Proof Sketch]
    It is true.
\end{proof}

\begin{theorem}[Probabilistically Complete]
    ET-GBT is probabilistically complete.
\end{theorem}
\begin{proof}[Proof Sketch]
    Follows directly from GBT and correctness.
\end{proof}

\subsection{Asymptotic Optimality}
\qh{Not sure if we can show this really}

We first show that the cost function in \eqref{eq:costfunction} satisfies the conditions for an admissible cost function according to \cite{Papadopoulos2014} for asymptotic near-optimality of sampling-based planning algorithms that sample the control space. It is easy to see that the cost function satisfies additivity, monotinicity, and non-degeneracy. In the following, we prove that the cost function is Lipschitz continuous in the control input ($\delta$).

% \begin{lemma}[Additivity]
%     \eqref{eq:costfunction} is additive.
% \end{lemma}
% \begin{proof}
%     Pretty straightforward. Cost function is a sum of stage costs at each time step.
% \end{proof}

% \begin{lemma}[monotonicity]
%     \eqref{eq:costfunction} is monotonically increasing.
% \end{lemma}
% \begin{proof}
%     Pretty straightforward. Cost function at each time step is $\geq 0$.
% \end{proof}

% \begin{lemma}[Non-degeneracy]
%     \eqref{eq:costfunction} is non-degenerate.
% \end{lemma}
% \begin{proof}
%     Proof is coming soon to a theater near you.
% \end{proof}

\begin{lemma}[Lipschitz Continuous]
    \eqref{eq:costfunction} is Lipschitz Continuous.
\end{lemma}
\begin{proof}
\qh{Still working on this}
It is enough to show the lipschitz continuity of one time step, since the cost function is a sum of stage costs at each time step.
    \begin{align*}
        J = \sum_{t=0}^{N}\Gamma(\delta_t) = \sum_{t=0}^{N} (1 - [1 - 2Q(\delta_t)]^m)
    \end{align*}
    For $\delta \in \positivereals$, we see that $\Gamma(\delta_t)$ is everywhere differentiable, and also that $J_t$ has a bounded first derivative, since $\delta \in \positivereals$. Therefore, it is Lipschitz continuous in $\delta$ according to \cite{nobody}.
\end{proof}

\begin{theorem}
    \qh{placeholder} ET-GBT with planners that sample the control space are asymptotically optimal for Problem~\ref{sec:problem}.
\end{theorem}
\begin{proof}
    \qh{How confident are we that this is true?}
    \qh{Maybe we can claim this for some starting values of $\Sigma$ and $\Lambda$, or locally}
    Smooth shifts in $\delta$ cause smooth shifts in the upper bound of the covariance, according to \eqref{eq:upperboundsigma} and \eqref{eq:upperboundlambda}. Thus, covariance upper bound \eqref{eq:upperboundcovariance} is Lipschitz continuous. Thus, smooth shifts in the state distribution causes smooth variations in $\Gamma(\delta)$. 
    
    Thus, sampling-based tree search motion planners that sample control inputs, such as SST*, are asymptotically optimal.
\end{proof}

% \begin{proof}
%     \qh{Work in progress... Check inequality signs. Only works for $\delta \in (c, \infty)$.}
%     It is enough to show the lipschitz continuity of one time step, since the cost function is a sum of stage costs at each time step.
%     \begin{align*}
%         J_t = \Gamma(\delta) = 1 - [1 - 2Q(\delta)]^m\\
%     \end{align*}
%     We seek to show that there exists a real constant $K \geq 0$ such that for all $\delta_1, \delta_2 \in (c, \infty)$ for $c > 0$,
%     \begin{align}
%         |\Gamma(\delta_1) - \Gamma(\delta_2)| &\leq K|\delta_1 - \delta_2|
%     \end{align}
    
%     \begin{align*}
%         |\Gamma(\delta_1) - \Gamma(\delta_2)| 
%         &= |(1 - [1 - 2Q(\delta_1)]^m - (1 - [1 - 2Q(\delta_2)]^m)|\\
%         &= |[1 - 2Q(\delta_1)]^m  - [1 - 2Q(\delta_2)]^m|\\
%         &< |1^m - 0^m| \text{ since } 0 < 2Q(\delta) < 1\\
%         &\leq \frac{1}{c}|\delta_1 - \delta_2|
%     \end{align*}
% \end{proof}

% \begin{proof}[\qh{Using continuous differentiability, not completed}]
%     We first show that $J$ is a differentiable and continuous function.
    
%     All power functions are continuous, and $Q$ is continuous...
%     Composition of two continuous function is continuous.
    
%     $J$ is differentiable, composition of two differentiable functions is differentiable. $Q$ is differentiable since it is defined by an integral... The power $m$ is also differentiable...
    
%     J has a bounded first derivative.
    
%     By the mean value theorem, we can show that it is lipschitz.
% \end{proof}

% \begin{proof}
%     Differentiable function is lipschitz on any interval on which its derivative is bounded
% \end{proof}

==> sections/ETBounds.tex <==
In this section, we present a novel method to predict the state distribution offline under an ET filter. The resulting distribution can be used to check the validity of the safety constraints.  Based on this method, we devise the planning algorithm in Sec. \ref{sec:ET-GBT}.

A key requirement for the method of belief prediction in Sec.~\ref{sec:KFpropagation} is that the distribution over state estimates, $\hat{x}_k$, is Gaussian, and defined by $\hat{x}_k \sim \mathcal{N}(\check{x}_k, \Lambda_k)$. When this distribution is known, it can be used to represent the joint distribution over $x_k$ and $\hat{x}_k$, which can in turn be marginalized to obtain the expected distribution over states, $x_k \sim \textbf{b}(x_k)=\mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$. This marginal is then used to evaluate the chance constraints in \eqref{eq:cc-obs} and \eqref{eq:cc-goal} offline.

Unfortunately, under ET estimation the covariance is updated under two randomly switching modes (according to $\gamma_k=0$ or $\gamma_k=1$), which means that the methods described in Sec. III.A cannot be directly applied to ET estimation. If the trigger $\gamma_k$ is treated as an unknown random variable, then the expected belief must be taken with respect to all possible $\gamma_k$, and is not Gaussian. However, if $\gamma_k$ is assumed to be given, then the distribution over $\hat{x}_k$ is Gaussian. This can be seen by examining the ET estimation update in \eqref{eq:ETaposterioriUpdate}: when $\gamma_k$ is given, the conditional dependency of $\hat{x}_k$ on $\gamma_k$ vanishes and the Gaussian property is preserved during the update. The mean and covariance can be obtained by evaluating $\mathbb{E}[\hat{x}_k]=\check{x}_k$ and $\mathbb{E}[(\hat{x}_k-\check{x}_k)(\hat{x}_k-\check{x}_k)^T]=\Lambda_k$ respectively. The resulting distribution $x_k \sim \mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$ can then be calculated, with $\Sigma_k$ given by the ET update in \eqref{eq:ETaposterioriUpdate} and $\Lambda_k$ given by: 
\begin{align}
\label{eq:ETcovupdate}
    \Lambda_k &= (A-BK)\Lambda_{k-1}(A-BK)^T + \gamma_k L_k C \Sigma_k^-.
\end{align}
The assumption that $\gamma_k$ is given is significant. Instead of taking the expected belief with respect to all possible $\gamma_k$, we assume a realization of some specific sequence of $\gamma_k$. However, if we are only concerned with bounding the probability of being within some region, this assumption can be easily accommodated. We simply need to determine the triggering condition that results in the expected belief with the highest, or lowest, probability of being in that region. 

It is intuitive to consider the following discussion from the perspective of risk. In robotics, we generally consider higher uncertainty as producing higher risk, or higher probability of violating safety constraints. While this is not technically true for certain situations, e.g., a tight distribution in close proximity to a small obstacle, it is reasonable for many robotics problems. So, for our problem we seek to determine the largest possible covariance, which  results in the highest probability of violating the safety constraint. If the safety constraint is satisfied for this worst case belief, then it must also be satisfied for all possible beliefs.

Consider the case for an arbitrary Gaussian belief $b(x)$ and some region $\mathcal{A} \subseteq \mathcal{X}$, where we require $P(x\in\mathcal{A})<p_\mathcal{A}$. We make the assumption that if the covariance of $b(x)$ satisfies the constraint, then any Gaussian belief with smaller covariance also satisfies the constraint, formally:
\begin{assumption}
    \label{as: covariance decrease CC better}
    If $x_a \sim b_a = \mathcal{N}(\mu, C_a)$, $x_b \sim b_b = \mathcal{N}(\mu, C_b)$, and $C_a > C_b$, then $P(x_a \in \mathcal{A}) < p_\mathcal{A} \implies P(x_b \in \mathcal{A}) < p_\mathcal{A}; \forall x \in \mathcal{X}$. 
\end{assumption}
Note that for matrices $\mathcal{X}, \mathcal{Y} \in \mathbb{R}^{n \times n}$, $\mathcal{X}>\mathcal{Y}$ implies $\mathcal{X}-\mathcal{Y}$ is positive definite and $\mathcal{X}\geq\mathcal{Y}$ means $\mathcal{X}-\mathcal{Y}$ is positive semi-definite. With this, it is only necessary to check the triggering sequence that results in the largest possible covariance, since we know that all other sequences (which necessarily result in smaller covariances) must also satisfy the constraint according to Assumption \ref{as: covariance decrease CC better}.

For ET estimation, this means determining the largest covariance for a given $\delta_k$. Under Assumption \ref{as: covariance decrease CC better}, this ensures satisfaction of constraints \eqref{eq:cc-obs} and \eqref{eq:cc-goal}. This is accomplished by calculating the bounding covariance that subsumes all covariances produced by any triggering condition. 
%
%To obtain these bounds, 
We use a bounding method similar to the one described in \cite{Li2018}. 

Let the scalar constants $\underline{a}, \bar{a}, \underline{k}, \bar{k}, \underline{c}, \bar{c},\underline{q}, \bar{q}$, $\underline{r}, \bar{r} \in \mathbb{R}_{>0}$ define bounds such that
\begin{equation}
\label{eq:SysBoundAssumptions}
\begin{split}
    &\underline{a}^2 I_n \leq A A^T \leq \bar{a}^2 I_n, \qquad \underline{c}^2 I_m \leq C C^T \leq \bar{c}^2 I_m, \\
    % \nonumber
    &\underline{k}^2 I_n \leq (A -BK)(A-BK)^T \leq \bar{k}^2, \\
    % \nonumber
    &\underline{q} I_n \leq Q \leq \bar{q} I_n,  \qquad \qquad\; \underline{r}I_m \leq R \leq \bar{r} I_m
    % \nonumber
\end{split}
\end{equation}
The existence of these positive bounds requires that the eigenvalues of $A$, $(A-BK)$, and $CC^T$ be real.

\begin{theorem}
    \label{theorem:covariance-bound}
    The predicted belief for ET estimation is given by $\textbf{b}(x_k)=\mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$, where the covariance $\Sigma_k+\Lambda_k$ is recursively updated according to \eqref{eq:ETcovupdate}. This covariance is recursively bounded by
    \begin{equation}
        \label{eq:upperboundcovariance}
        \Lambda_k + \Sigma_k \leq (\bar{\lambda}_k + \bar{p}_k) I_n
    \end{equation}
    where $\bar{\lambda}_k,\bar{p}_k \in \mathbb{R}_{\geq 0}$ are given by:
    \begin{align}
        % \label{eq:upperboundlambda}
        &\bar{\lambda}_k = \bar{k}^2\bar{\lambda}_{k-1} + \frac{\bar{c}^2\left( \bar{p}_{k-1}\bar{a}^2 + \bar{q} \right)^2}{\underline{c}^2\left( \underline{p}_{k-1}\underline{a}^2 + \underline{q} \right) + \underline{r}} \nonumber\\
        % \label{eq:upperboundsigma}
        &\bar{p}_k = \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1}
        \nonumber
    \end{align}
with $\underline{p}_k= \left( 1/\underbar{q} + \bar{c}^2/\underbar{r} \right)^{-1}$.
The bounds are initialized as:
\begin{align*}
    &\bar{\lambda}_0 = \max \left(Eigenval\left(\Lambda_0\right)\right), \\
    &\bar{p}_0 = \max\left(Eigenval\left(\Sigma_0\right)\right), \; \underline{p}_0 = \min\left(Eigenval\left(\Sigma_0\right)\right).
\end{align*}
% where $Eval(\cdot)$ refers to the eigenvalues. 

\end{theorem}
\emph{Proof Sketch:} We follow the techniques developed in \cite{Li2018}, which relies on matrix manipulations of the inverse form of the covariance update. A detailed proof is provided in the extended version of this paper \cite{Theurkauf2022extended}.
%\emph{Proof Sketch} We follow the techniques developed in \cite{Li2018}, which relies on matrix manipulations of the inverse form of the covariance update. For both $\Lambda_k$ and $\Sigma_k$ we examined the upper and lower bounds for the two possible cases for the update, $\gamma_k=0$ and $\gamma_k=1$, and determined the lowest lower bound and highest upper bound. This provides the comprehensive bounds in \eqref{eq:upperboundlambda}, \eqref{eq:upperboundsigma}, and \eqref{eq:lowerboundsigma}. A detailed proof is provided in the extended version of this paper: \at{make extended version...}.


%%%%%%%%%% Will return to workshop this proof after ICRA deadline (efficient)
\begin{comment}

We also rely on the following lemmas:
\ml{These lemmas should be in the prelims section.  Maybe add a subsection to that section called something like ``Definite Matrices and Bounds''???}
\begin{lemma}
    Assume that $A,B\in\mathbb{R}^{n\times n}$, if $A>0$ and $B\geq0$, then
    \ml{are these $A$ and $B$ matrices different from the ones in the dynamics?}
    \begin{equation}
        A^{-1}\geq(A+B)^{-1}
    \end{equation}
\end{lemma}
\begin{lemma}
    Assume that $A\in\mathbb{R}^{n\times n}$ is bounded such that $A\leq \bar{a}I_n$, then $A^{-1}\geq 1/\bar{a} I_n$
    \ml{same $A$ as in the dynamics?}
\end{lemma}

\qh{Can we have equations for the lower bound as well? Since we have to maintain them for ET-GBT}\at{Do we actually use the lower bound on $\Lambda$? I thought we only need the upper for collision checking, and the nearest node uses the upper bound?}\qh{Yeah I think it should be fine, but because in the GBT part I wrote that we maintain both the upper and lower bounds (4 values)}

\ml{what's the intuition of the following theorem?  Tell the reader what to expect from the theorem.}

\ml{I think the theorem statement is wrong... I'm guessing you want to say that predicted covariance of the
state belief at time $k$ under ET Filter can be recursively bounded by... ? Also, need to to define $\bar{\lambda}_0,\bar{p}_0$
}

\begin{theorem}
    \label{theorem:covariance-bound}
    There always exists an upper bound
    \ml{positive scalars?}
    , $\bar{\lambda}_k \in \mathbb{R}_{\geq 0}$, and upper bound $\bar{p}_k \in \mathbb{R}_{\geq 0}$ such that $\Lambda_k+\Sigma_k$ satisfies:
    \begin{equation}
        \label{eq:upperboundcovariance}
        \Lambda_k + \Sigma_k \leq (\bar{\lambda}_k + \bar{p}_k) I_n
    \end{equation}
    \ml{aren't $\Lambda,\Sigma > 0$ (PD)?}
    where
    \begin{align}
        \label{eq:upperboundlambda}
        &\bar{\lambda}_k = \bar{k}^2\bar{\lambda}_{k-1} + \frac{\bar{c}^2\left( \bar{p}_{k-1}\bar{a}^2 + \bar{q} \right)^2}{\underline{c}^2\left( \underline{p}_{k-1}\underline{a}^2 + \underline{q} \right) + \underline{r}}
    \end{align}
    \begin{align}
        \label{eq:upperboundsigma}
        &\bar{p}_k = \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1}
    \end{align}
    and
    \begin{equation}
    \label{eq:lowerboundsigma}
        \underline{p}_k= \left( \frac{1}{\underbar{q}} + \frac{\bar{c}^2}{\underbar{r}} \right)^{-1}
    \end{equation}

\end{theorem}

\begin{proof}
\ml{I didn't check the proof yet!}
We first derive a bound for $\Lambda_k$ such that $\Lambda_k \leq \bar{\lambda}_k I_n$. Consider the case $\gamma_k=1$. The update equation can be written as:
\begin{align}
\label{eq:lambdaUpdateGamma0}
    \Lambda_k &= (A-BK)\Lambda_{k-1}(A-BK)^T \\
    & + \Sigma_k^- C^T(C\Sigma_k^- C^T + R)^{-1} C \Sigma_k^-.
\end{align}
The first term can be simply bounded as $(A-BK)\Lambda_{k-1}(A-BK)^T\leq\bar{k}^2\bar{\lambda}_{k-1}$. Now consider the second term. Begin by deriving bounds on $\Sigma_k^-$: from \eqref{eq:ETcovupdate}, we can generate the bounds
\begin{equation}
    \underline{a}^2\underline{p}_{k-1} + \underline{q} \leq \Sigma_k^- \leq \bar{a}^2\bar{p}_{k-1} + \bar{q} 
\end{equation}
where $\underline{p}_k$ and $\bar{p}_k$ represent lower and upper bounds on $\Sigma_k$ such that $\underline{p}_k \leq \Sigma_k \leq \bar{p}_k$. Additionally, we see that $C\Sigma_k^- C^T + R \geq \underline{c}^2(\underline{p}_{k-1}\underline{a}^2 + \underline{q})$, and by applying the inverse, we obtain $(C\Sigma_k^- C^T + R)^{-1} \leq (\underline{c}^2(\underline{p}_{k-1}\underline{a}^2 + \underline{q}))^{-1}$. Combining these yields the bound in \eqref{eq:upperboundlambda}.  This clearly subsumes the upper bound for the case $\gamma_k=0$, which only contains the first term in \eqref{eq:lambdaUpdateGamma0}, yielding $\Lambda_{k,\gamma_k=0} \leq \bar{k}^2\bar{\lambda}_{k-1} I_n$.

Next, we can use a similar reasoning to generate bounds on $\Sigma_k$. Global bounds must consider the lower and upper bounds for each case, $\gamma_k=1$ and $\gamma_k=0$. For the case $\gamma_k=1$, \eqref{eq:sigma_k} becomes the standard KF equations. Therefore, the upper and lower bounds for the case $\gamma_k=1$ are the same KF bounds derived in \cite{Li2016}: 
\begin{equation}
\left( \frac{1}{\underbar{q}} + \frac{\bar{c}^2}{\underbar{r}} \right)^{-1} I_n \leq \Sigma_{k,\gamma_k=1} \leq \left(\bar{p}_{k-1}\bar{a}^2 + \bar{q}\right)I_n
\end{equation}

We derive the bounds for the case $\gamma_k=0$ based on the inverse form of the covariance update equation for $\gamma_k=0$:
\begin{equation}
\begin{split}
    &\Sigma_{k,\gamma_k=0} = \\
    &\left( \left(\Sigma_k^-\right)^{-1} + \beta C_k^T \left(  R_k + \left(1-\beta\right)C_k\Sigma_k^- C_k^T \right)^{-1} C_k \right)^{-1}
\end{split}
\end{equation}
Under straightforward manipulation this yields the bounds:
\begin{align}
    &\left( \frac{1}{\underbar{q}} + \frac{\beta\bar{c}^2}{\underbar{r} + (1-\beta)\underline{c}^2\underbar{q}} \right)^{-1} I_n \leq \Sigma_{k,\gamma_k=0} \\
    & \leq \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1} I_n
\end{align}
Note that the lower bound for the case $\gamma_k=1$ subsumes the lower bound for $\gamma_k=0$, yielding the true lower bound in \eqref{eq:lowerboundsigma}. Similarly, the upper bound for $\gamma_k=0$ subsumes the upper bound for $\gamma_k=1$, yielding the true upper bound in \eqref{eq:upperboundsigma}.

Finally, we can bound the sum of the covariances $\Sigma_k + \Lambda_k$ by the sum of their respective upper bounds: $\Sigma_k + \Lambda_k \leq (\bar{p}_k + \bar{\lambda}_k) I_n$.
\end{proof}
\end{comment}


==> sections/ETBounds_final.tex <==
In this section, we present a novel method to predict the state distribution offline under an ET filter. The resulting distribution can be used to check the validity of the safety constraints.  Based on this method, we devise a planning algorithm in Sec. \ref{sec:ET-GBT}.

A key requirement for the method of belief prediction in Sec.~\ref{sec:KFpropagation} is that the distribution over state estimates, $\hat{x}_k$, is Gaussian, and defined by $\hat{x}_k \sim \mathcal{N}(\check{x}_k, \Lambda_k)$. When this distribution is known, it can be used to represent the joint distribution over $x_k$ and $\hat{x}_k$, which can in turn be marginalized to obtain the expected distribution over states, $x_k \sim \textbf{b}(x_k)=\mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$. This marginal is then used to evaluate the chance constraints in \eqref{eq:cc-obs} and \eqref{eq:cc-goal} offline.

Unfortunately, under ET estimation the covariance is updated under two randomly switching modes (according to $\gamma_k=0$ or $\gamma_k=1$), which means that the methods described in Sec. III.A cannot be directly applied to ET estimation. If the trigger $\gamma_k$ is treated as an unknown random variable, then the expected belief must be taken with respect to all possible $\gamma_k$, and is not Gaussian. However, if $\gamma_k$ is assumed to be given, then the distribution over $\hat{x}_k$ is Gaussian. This can be seen by examining the ET estimation update in \eqref{eq:ETaposterioriUpdate}: when $\gamma_k$ is given, the conditional dependency of $\hat{x}_k$ on $\gamma_k$ vanishes and the Gaussian property is preserved during the update. The mean and covariance can be obtained by evaluating $\mathbb{E}[\hat{x}_k]=\check{x}_k$ and $\mathbb{E}[(\hat{x}_k-\check{x}_k)(\hat{x}_k-\check{x}_k)^T]=\Lambda_k$ respectively. The resulting distribution $x_k \sim \mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$ can then be calculated, with $\Sigma_k$ given by the ET update in \eqref{eq:ETaposterioriUpdate} and $\Lambda_k$ given by: 
\begin{align}
\label{eq:ETcovupdate}
    \Lambda_k &= (A-BK)\Lambda_{k-1}(A-BK)^T + \gamma_k L_k C \Sigma_k^-.
\end{align}
The assumption that $\gamma_k$ is given is significant. Instead of taking the expected belief with respect to all possible $\gamma_k$, we assume a realization of some specific sequence of $\gamma_k$. However, if we are only concerned with bounding the probability of being within some region, this assumption can be easily accommodated. We simply need to determine the triggering condition that results in the expected belief with the highest or lowest probability of being in that region. 

% \at{
While the expectation of triggering at any given time step is  easy to calculate, the corresponding expected belief is not. However, because we are considering a chance constraint, it is sufficient to only consider an upper bounding belief, which  subsumes all covariances produced by any triggering condition. This bound can be used for collision checking as described in Section \ref{sec:validityChecking} to guarantee satisfaction of the chance constraints.
% }
%
%To obtain these bounds, 
We use a bounding method similar to the one described in \cite{Li2018}. 

Let the scalar constants $\underline{a}, \bar{a}, \underline{k}, \bar{k}, \underline{c}, \bar{c},\underline{q}, \bar{q}$, $\underline{r}, \bar{r} \in \mathbb{R}_{>0}$ define bounds such that
\begin{equation}
\label{eq:SysBoundAssumptions}
\begin{split}
    &\underline{a}^2 I_n \leq A A^T \leq \bar{a}^2 I_n, \qquad \underline{c}^2 I_m \leq C C^T \leq \bar{c}^2 I_m, \\
    % \nonumber
    &\underline{k}^2 I_n \leq (A -BK)(A-BK)^T \leq \bar{k}^2, \\
    % \nonumber
    &\underline{q} I_n \leq Q \leq \bar{q} I_n,  \qquad \qquad\; \underline{r}I_m \leq R \leq \bar{r} I_m,
    % \nonumber
\end{split}
\end{equation}
where $I_m$ is the $m\times m$ identity matrix, and inequality relation $\textit{X} \geq \textit{Y}$ for square matrices $\textit{X}$ and $\textit{Y}$ implies $\textit{X}-\textit{Y}$ is positive semi-definite. 
Note that the existence of these positive bounds requires that the eigenvalues of $A$, $(A-BK)$, and $CC^T$ be real.  Based on these parameters, we derive an upper bound for the covariance of the belief in the theorem below.

\begin{theorem}
    \label{theorem:covariance-bound}
    Consider the predicted belief for ET estimation given by $\textbf{b}(x_k)=\mathcal{N}(\check{x}_k,\Sigma_k+\Lambda_k)$, where the covariance $\Sigma_k+\Lambda_k$ is recursively updated according to \eqref{eq:ETcovupdate}. Then, this covariance can be recursively bounded by
    \begin{equation}
        \label{eq:upperboundcovariance}
        \Lambda_k + \Sigma_k \leq (\bar{\lambda}_k + \bar{p}_k) I_n
    \end{equation}
    where $\bar{\lambda}_k,\bar{p}_k \in \mathbb{R}_{\geq 0}$ are given by
    \begin{align}
        % \label{eq:upperboundlambda}
        &\bar{\lambda}_k = \bar{k}^2\bar{\lambda}_{k-1} + \frac{\bar{c}^2\left( \bar{p}_{k-1}\bar{a}^2 + \bar{q} \right)^2}{\underline{c}^2\left( \underline{p}_{k-1}\underline{a}^2 + \underline{q} \right) + \underline{r}} \nonumber\\
        % \label{eq:upperboundsigma}
        &\bar{p}_k = \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1}
        \nonumber
    \end{align}
with $\underline{p}_k= \left( 1/\underbar{q} + \bar{c}^2/\underbar{r} \right)^{-1}$.
The bounds are initialized as:
\begin{align*}
    &\bar{\lambda}_0 = \max \left(Eigenval\left(\Lambda_0\right)\right), \\
    &\bar{p}_0 = \max\left(Eigenval\left(\Sigma_0\right)\right), \; \underline{p}_0 = \min\left(Eigenval\left(\Sigma_0\right)\right).
\end{align*}
% where $Eval(\cdot)$ refers to the eigenvalues. 

\end{theorem}
\emph{Proof Sketch:} We follow the techniques developed in \cite{Li2018}.
%, which relies on matrix manipulations of the inverse form of the covariance update. 
A detailed proof is provided in the extended version of this paper \cite{Theurkauf2022extended}.
%\emph{Proof Sketch} We follow the techniques developed in \cite{Li2018}, which relies on matrix manipulations of the inverse form of the covariance update. For both $\Lambda_k$ and $\Sigma_k$ we examined the upper and lower bounds for the two possible cases for the update, $\gamma_k=0$ and $\gamma_k=1$, and determined the lowest lower bound and highest upper bound. This provides the comprehensive bounds in \eqref{eq:upperboundlambda}, \eqref{eq:upperboundsigma}, and \eqref{eq:lowerboundsigma}. A detailed proof is provided in the extended version of this paper: \at{make extended version...}.


%%%%%%%%%% Will return to workshop this proof after ICRA deadline (efficient)
\begin{comment}

We also rely on the following lemmas:
\ml{These lemmas should be in the prelims section.  Maybe add a subsection to that section called something like ``Definite Matrices and Bounds''???}
\begin{lemma}
    Assume that $A,B\in\mathbb{R}^{n\times n}$, if $A>0$ and $B\geq0$, then
    \ml{are these $A$ and $B$ matrices different from the ones in the dynamics?}
    \begin{equation}
        A^{-1}\geq(A+B)^{-1}
    \end{equation}
\end{lemma}
\begin{lemma}
    Assume that $A\in\mathbb{R}^{n\times n}$ is bounded such that $A\leq \bar{a}I_n$, then $A^{-1}\geq 1/\bar{a} I_n$
    \ml{same $A$ as in the dynamics?}
\end{lemma}

\qh{Can we have equations for the lower bound as well? Since we have to maintain them for ET-GBT}\at{Do we actually use the lower bound on $\Lambda$? I thought we only need the upper for collision checking, and the nearest node uses the upper bound?}\qh{Yeah I think it should be fine, but because in the GBT part I wrote that we maintain both the upper and lower bounds (4 values)}

\ml{what's the intuition of the following theorem?  Tell the reader what to expect from the theorem.}

\ml{I think the theorem statement is wrong... I'm guessing you want to say that predicted covariance of the
state belief at time $k$ under ET Filter can be recursively bounded by... ? Also, need to to define $\bar{\lambda}_0,\bar{p}_0$
}

\begin{theorem}
    \label{theorem:covariance-bound}
    There always exists an upper bound
    \ml{positive scalars?}
    , $\bar{\lambda}_k \in \mathbb{R}_{\geq 0}$, and upper bound $\bar{p}_k \in \mathbb{R}_{\geq 0}$ such that $\Lambda_k+\Sigma_k$ satisfies:
    \begin{equation}
        \label{eq:upperboundcovariance}
        \Lambda_k + \Sigma_k \leq (\bar{\lambda}_k + \bar{p}_k) I_n
    \end{equation}
    \ml{aren't $\Lambda,\Sigma > 0$ (PD)?}
    where
    \begin{align}
        \label{eq:upperboundlambda}
        &\bar{\lambda}_k = \bar{k}^2\bar{\lambda}_{k-1} + \frac{\bar{c}^2\left( \bar{p}_{k-1}\bar{a}^2 + \bar{q} \right)^2}{\underline{c}^2\left( \underline{p}_{k-1}\underline{a}^2 + \underline{q} \right) + \underline{r}}
    \end{align}
    \begin{align}
        \label{eq:upperboundsigma}
        &\bar{p}_k = \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1}
    \end{align}
    and
    \begin{equation}
    \label{eq:lowerboundsigma}
        \underline{p}_k= \left( \frac{1}{\underbar{q}} + \frac{\bar{c}^2}{\underbar{r}} \right)^{-1}
    \end{equation}

\end{theorem}

\begin{proof}
\ml{I didn't check the proof yet!}
We first derive a bound for $\Lambda_k$ such that $\Lambda_k \leq \bar{\lambda}_k I_n$. Consider the case $\gamma_k=1$. The update equation can be written as:
\begin{align}
\label{eq:lambdaUpdateGamma0}
    \Lambda_k &= (A-BK)\Lambda_{k-1}(A-BK)^T \\
    & + \Sigma_k^- C^T(C\Sigma_k^- C^T + R)^{-1} C \Sigma_k^-.
\end{align}
The first term can be simply bounded as $(A-BK)\Lambda_{k-1}(A-BK)^T\leq\bar{k}^2\bar{\lambda}_{k-1}$. Now consider the second term. Begin by deriving bounds on $\Sigma_k^-$: from \eqref{eq:ETcovupdate}, we can generate the bounds
\begin{equation}
    \underline{a}^2\underline{p}_{k-1} + \underline{q} \leq \Sigma_k^- \leq \bar{a}^2\bar{p}_{k-1} + \bar{q} 
\end{equation}
where $\underline{p}_k$ and $\bar{p}_k$ represent lower and upper bounds on $\Sigma_k$ such that $\underline{p}_k \leq \Sigma_k \leq \bar{p}_k$. Additionally, we see that $C\Sigma_k^- C^T + R \geq \underline{c}^2(\underline{p}_{k-1}\underline{a}^2 + \underline{q})$, and by applying the inverse, we obtain $(C\Sigma_k^- C^T + R)^{-1} \leq (\underline{c}^2(\underline{p}_{k-1}\underline{a}^2 + \underline{q}))^{-1}$. Combining these yields the bound in \eqref{eq:upperboundlambda}.  This clearly subsumes the upper bound for the case $\gamma_k=0$, which only contains the first term in \eqref{eq:lambdaUpdateGamma0}, yielding $\Lambda_{k,\gamma_k=0} \leq \bar{k}^2\bar{\lambda}_{k-1} I_n$.

Next, we can use a similar reasoning to generate bounds on $\Sigma_k$. Global bounds must consider the lower and upper bounds for each case, $\gamma_k=1$ and $\gamma_k=0$. For the case $\gamma_k=1$, \eqref{eq:sigma_k} becomes the standard KF equations. Therefore, the upper and lower bounds for the case $\gamma_k=1$ are the same KF bounds derived in \cite{Li2016}: 
\begin{equation}
\left( \frac{1}{\underbar{q}} + \frac{\bar{c}^2}{\underbar{r}} \right)^{-1} I_n \leq \Sigma_{k,\gamma_k=1} \leq \left(\bar{p}_{k-1}\bar{a}^2 + \bar{q}\right)I_n
\end{equation}

We derive the bounds for the case $\gamma_k=0$ based on the inverse form of the covariance update equation for $\gamma_k=0$:
\begin{equation}
\begin{split}
    &\Sigma_{k,\gamma_k=0} = \\
    &\left( \left(\Sigma_k^-\right)^{-1} + \beta C_k^T \left(  R_k + \left(1-\beta\right)C_k\Sigma_k^- C_k^T \right)^{-1} C_k \right)^{-1}
\end{split}
\end{equation}
Under straightforward manipulation this yields the bounds:
\begin{align}
    &\left( \frac{1}{\underbar{q}} + \frac{\beta\bar{c}^2}{\underbar{r} + (1-\beta)\underline{c}^2\underbar{q}} \right)^{-1} I_n \leq \Sigma_{k,\gamma_k=0} \\
    & \leq \left( \frac{1}{\bar{p}_{k-1}\bar{a}^2 + \bar{q}} + \frac{\beta\underline{c}^2}{\bar{r} + \left( 1-\beta \right)\bar{c}^2\left( \bar{a}^2\bar{p}_{k-1}+\bar{q}\right) } \right)^{-1} I_n
\end{align}
Note that the lower bound for the case $\gamma_k=1$ subsumes the lower bound for $\gamma_k=0$, yielding the true lower bound in \eqref{eq:lowerboundsigma}. Similarly, the upper bound for $\gamma_k=0$ subsumes the upper bound for $\gamma_k=1$, yielding the true upper bound in \eqref{eq:upperboundsigma}.

Finally, we can bound the sum of the covariances $\Sigma_k + \Lambda_k$ by the sum of their respective upper bounds: $\Sigma_k + \Lambda_k \leq (\bar{p}_k + \bar{\lambda}_k) I_n$.
\end{proof}
\end{comment}


==> sections/preliminaries.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Belief Prediction under Kalman Filter}
\label{sec:KFpropagation}

For a linearizable and controllable system operating under a standard KF, \cite{Bry2011} presents a method to forecast the belief over the state while accounting for the fact that the measurements are unknown random variables \emph{a priori}. This \emph{expected belief}, $\textbf{b}(x_k)$, is defined with respect to all possible measurements as:
\begin{align}
    \label{eq: expected belief}
    \textbf{b}(x_k) = \mathbb{E}_Y[b(x_k \mid x_0, y_{0:k})]
    = \int_{y_{0:k}} \hspace{-3mm} b(x_k \mid x_0, y_{0:k}) pr(y_{0:k})dy \nonumber
\end{align}
This forecast enables the evaluation of the chance constraints.

For a given nominal trajectory, $\check{X}_0^T=(\check{x}_0, \ldots, \check{x}_T)$,  the expected belief $\textbf{b}(x_k)=\mathcal{N}(\check{x}_k, \Sigma_k+\Lambda_k)$, can be recursively calculated from an initial belief $b(x_0)$ using the belief propagation method from \cite{Bry2011}:
\begin{align}
    \Sigma_k^- &= A\Sigma_{k-1}A^T + Q, \quad \Sigma_k = \Sigma_k^- - L_k C\Sigma_k^-, \\
    \Lambda_k &= (A-BK)\Lambda_{k-1}(A-BK)^T + L_k C \Sigma_k^-,
\end{align}
where $\Sigma_k$ is the online uncertainty given by the KF, and $\Lambda_k$ is covariance of the forecasted state estimates $\hat{x}_k$ (note that $\hat{x}_k$ is a random variable offline). Intuitively, this distribution can be thought of as the sum of the online estimation error and the forecasted uncertainty from not-yet-known measurements that the system receives during execution.  In this work, we develop a method of forecasting belief under an ET Filter.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
\subsection{MMSE Filter for Event-triggered Estimation}
\label{sec:ETfilter}

For state estimation,
we use the triggering scheme described in \cite{Wu2013}, which is based on the KF innovation. Recall that the trigger, $\gamma_k$, depends on the triggering threshold $\delta_k$.
%, and that $\gamma_k = 1$ indicates that measurement $y_k$ is sent, and $\gamma_k=0$ otherwise
According to the MMSE estimator in \cite{Wu2013}, the estimate of the state is Gaussian with \textit{a priori} update:
\begin{equation}
\label{eq:ETaprioriUpdate}
    \hat{x}_k^- = A \hat{x}_{k-1} + B u_k, \quad \Sigma_k^- = A \Sigma_{k-1} A^T + Q,
\end{equation}
and \textit{a posteriori} update given by:
\begin{align}
\label{eq:ETaposterioriUpdate}
    &\hat{x}_k = \hat{x}_k^- + \gamma_k L_k z_k, \quad z_k = y - C\hat{x}_k^- \\
    % &\Sigma_k = \gamma_k g(\Sigma_k^-,1) + (1-\gamma_k)g(\Sigma_k^-, \beta(\delta)).
    &\Sigma_k =  \Sigma_k^- - \Big[\gamma_k + (1-\gamma_k) \beta(\delta_k) \Big] L_k C\Sigma_k^-.
\end{align}
where 
% $g(\Sigma_k, {\beta(\delta)}) = \Sigma_k - \beta(\delta) L_k\Sigma_k C$, and 
$L_k=\Sigma_k^- C^T[C \Sigma_k^-C^T + R]^{-1}$ is the KF gain. The term ${\beta(\delta_k)}$ is a scalar multiplier that effectively attenuates the KF gain in the covariance update as a function of $\delta_k$, and is given by
\begin{equation}
\beta(\delta) = \frac{2}{\sqrt{2\pi}}\delta e^{-\frac{\delta^2}{2}}\left[ 1 - 2\mathcal{Q}(\delta) \right]^{-1},
\end{equation}
where
\begin{equation}
    \mathcal{Q}(\delta) \triangleq \int_\delta^{+\infty} \frac{1}{\sqrt{2\pi}} e^{-\frac{x^2}{2}}dx.
\end{equation}

The triggering condition takes the form: 
\begin{equation}
    \gamma_k = 
    \begin{cases}
    0 & \text{if $\|\epsilon_k\|_\infty\leq\delta_k$}\\
    1 & \text{otherwise},
    \end{cases}
\end{equation}
where 
% $\delta_k \in \positivereals$ is the triggering threshold, and 
$\epsilon_k$ is the Mahalanobis (whitening) transformation of the KF innovation, $z_k$.
% Now, consider the expectation defined in \eqref{eq:ExpectedCost}. 
Note that, because of the whitening transformation, $\epsilon_k$ is always distributed as a standard normal.  Hence, the expected value of $\gamma_k$
is solely dependent on $\delta_k$ and is given by $\Gamma(\delta_k)= 1-\left[ 1 - 2\mathcal{Q}(\delta_k)\right]^m$, where $m$ is the dimension of the measurement vector.

